On Time Domain Conformer Models for Monaural Speech Separation in Noisy Reverberant Acoustic Environments

Speech separation remains an important topic for multi-speaker technology researchers. Convolution augmented transformers (conformers) have performed well for many speech processing tasks but have been under-researched for speech separation. Most recent state-of-the-art (SOTA) separation models have been time-domain audio separation networks (TasNets). A number of successful models have made use of dual-path (DP) networks which sequentially process local and global information. Time domain conformers (TD-Conformers) are an analogue of the DP approach in that they also process local and global context sequentially but have a different time complexity function. It is shown that for realistic shorter signal lengths, conformers are more efficient when controlling for feature dimension. Subsampling layers are proposed to further improve computational efficiency. The best TD-Conformer achieves 14.6 dB and 21.2 dB SISDR improvement on the WHAMR and WSJ0-2Mix benchmarks, respectively.

==> complexity_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!ht]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|}
\hline
\textbf{Layer} & \textbf{Local complexity}                     & \textbf{Global complexity}                             \\ \hline
Conformer      & $\frac{L_\vek{x}}{2^S} \left(PB+B^2\right)$    & $\frac{L_\vek{x}^2}{2^{2S}}B+B^2\frac{L_\vek{x}}{2^S}$ \\\hline
DP Transformer & $\left(\frac{L_\vek{x}}{2P}+\frac{P}{2}\right) \left(P^2B+B^2P\right)$ & $\frac{L_\vek{x}}{4P^2}B+B^2\frac{L_\vek{x}}{2P}$      \\ \hline
\end{tabular}%
}
\caption{Comparison of time-complexities for local and global parts of the conformer and dual-path transformer layers.}
\label{tab:tc_comp}
\end{table}
